Cosmological simulations of the generation of cluster-scale radio emission from turbulent re-acceleration

Context. The recent discovery of so-called mega radio halos as a new class of diffuse, steep-spectrum radio sources in clusters of galaxies has raised questions about the origin and the evolution of cluster-wide radio emission. Aims. We investigate whether the formation mechanisms of radio halos and mega radio halos differ, or whether they can be produced by different modalities of the same (re)acceleration mechanism. Here we present results of a cosmological simulation of a disturbed galaxy cluster, with the aim to study the origin of mega radio halos. Methods. We analysed the evolution of cosmic-ray electrons, subject to gains and losses using a Fokker-Planck solver. In particular, we included the effects of Adiabatic Stochastic Acceleration (ASA) which is caused by the stochastic interaction of cosmic rays with diffusing magnetic field lines in super-Alfvenic turbulence. Moreover, we included shock acceleration and the seeding of cosmic-ray electrons by galaxies. Results. Our simulations generate cluster-scale radio sources during mergers, with properties that are in agreement with those observed for real radio halos. Furthermore, we find evidence of additional emission on larger scales. This emission resembles the radial distribution and the spectrum of a mega radio halo, but only when viewed close to the merger axis. Conclusions. In our simulation, the mechanism responsible for the formation of diffuse radio emission, both in the form of classical and mega radio halos, is cosmic-ray re-acceleration by turbulence. This turbulence is more solenoidal and more subsonic in the classical radio halo region, than in the mega radio halo region.

==> 0_referee_report_with_replies.tex <==
We thank our Reviewer for his feedback on our work: it turned out to be extremely helpful.
In this revised version, we took into account all suggestions, and introduced longer and more detailed explanations of several crucial points. This resulted into a longer manuscript, including 4 new plots (arranged in new Fig. 3 and 6). 
All important modifications introduced in the manuscript are marked in boldface. Here below is our detailed list of answers to our Reviewer's comments.
We hope that this work can now be considered for publication.
Best regards
L. Beduzzi (on behalf of all coauthors).



=================================================

R:--- It is stressed on p. 4, and re-stressed on p. 6, that a fundamental finding (even a surprise?) here is that CR electrons live longer than expected (it is not entirely clear by whom this was expected, or on what grounds, maybe a reference would help?). 

A: This is indeed a key result of our paper, and in order to better show how this may revise the more classical estimates of the lifetime of radio emitting electrons in the ICM, we added a longer dedicated discussion in Sec.4, as well as a three panel Figure (new Fig. 6), which should best illustrate our result in a concise way. 


R: On p. 4, and then 5, this is explained by a balance of re-acceleration and loss time scales, gleaned from numerical measurements. Can some useful twiddle estimate be made here? If I assume such a balance, can I predict this result analytically? What would this imply for various scalings? Importantly, what would this imply for how fine-tuned this result is --- what would break it and how sensitive is the viability of such a balance to theoretical assumptions and numerical choices? I am not demanding a quantitative theory, just a back-of-a-napkin theoretical scoping out to match the numerical one reported here.

A: Similar as before: the new Fig.6 illustrates how the classical picture of the distribution of CR lifetimes in a cluster is changed if we include the new view of turbulent re-acceleration highlighted by our analysis. This has also led to a longer concluding discussion, in Sec.4.  

R:
--- Another important numerical finding seems to be that the CR electrons in MegaRH have been inside the Classical RH already, rather then accreting from outside. Again, can some useful twiddle estimate be made here, say, how long does a CR electron stay confined and so does it make sense to think of the MegaRH as a kind of atmosphere/corona through which these electrons are evaporating out? Does the size of the MegaRH make sense in that context?

A: We produced a new figure (Fig.3) to strengthen this point: it gives the evolution with time of the median distance of the families of tracers from the cluster centre, and it shows that the two family were almost at the same distance at all times, with the exception of the latest 1-2 Gyrs. 


R:--- Perhaps some brief discussion of why the Brunetti-Lazarian re-acceleration scheme should be used rather than something else? I know this is referred to previous literature, but for a busy astronomer who is prepared to read just this, can you make an elevator pitch for why this is the right physics to invoke (beyond just "we use it and it works fine").
A: We added a longer discussion of this in Sec.2.1 


R:
--- There is a reference to scale L in eq. 1 not mattering in a Kolmogorov V^3/L = const situation. Great, but is Kolmogorov incompressible turbulence actually what you have in there? What are the Mach numbers? Is there a spectrum of motions that at all resembles K41?
A: We added a longer comment on this at the end of Sec.2, in which we referred to our previous works on the issue. 



R: --- A significant model-dependent aspect seems to be the question of how CR electrons might diffuse and, therefore, whether the whole particle-tracking scheme followed here is sensible. Footnote 1 quotes a CR diffusion scale of < 100 pc but gives no explanation of how this obtained. Can you explain what is assumed and assess how sensitive your results are to that? There is a huge literature on CR confinement, both physics and modelling, so it would be useful to connect to that.
A: We addressed this issue, with a longer explanation and line showing the relative value of CR diffusion compared to other timescales, in Sec.4 and Fig.6.


Some minor issues:

R: On p. 2, they mention scaling up the organically created magnetic fields --- but they don't explain how, by how much, how these scaled-up fields are maintained etc. In footnote 1, there is an intimation that they are on microGauss level, and one can see that also in Fig 2a, but there's no detail. A bit more info would help.
A: We added a longer explanation about this procedure at the end of Sec.2. 



R: 
At the bottom of the left column of p. 2, there is an incomplete sentence: "The distribution of particles was created by sampling a fixed gas mass resolution of..." ---???
A: We fixed this in the revised draft, thanks.

R:
p. 5 major mergers ---> major merger; gas always keep ---> gas always keeps
A: done 



==> referee_report.tex <==
R:Referee
A:authors

R:  Line 23: The definition of $R_{500}$ is missing. 
A: Fixed with footnote 1, which also is used to define all other similar radii and masses quoted in the paper. 

R: Line 41: There are also works that refer to collisionless plasmas: Ha et al., 2021, ApJ, or a recent one in A&A Boula et al., 2024. These are related to particle pre-acceleration that can help to an efficient DSA. 
A: - We added a reference to additional works in the revised Introduction.

R: Line 121: Reference to the ENZO code is needed. 
A:Fixed. 

R: Line 171: Definition of the quantities (e.g., v_{gas}). 
A: Fixed

R: Line 179: Regarding DSA Qinj, in the work of Amano and Masahiro, 2022, ApJ, the theory of electron injection at an oblique shock of finite thickness is presented. Can the authors' Fokker-Planck method take into account the findings of SSDA? This could be a point of discussion for the publication, which is under preparation (Vazza et al., in prep).
A: We commented on this in the new draft. 

R: Line 183: Define the losses. 
A: Fixed 

R: Lines 198 / 224: ϕ=10{−6}: They mention the reason for choosing this number (injected into the highest gas density peak) in the conclusions. It might be helpful to mention this at the first point. 
A: Done 

R: Line 295: Consider adding an Appendix to show the Fokker-Planck equations in detail. This will be very useful for comparing terms and understanding the timescales, etc. - 
A: We addressed this suggestion by adding a short appendix explicilty showing the loss terms (the shock and turbulent acceleration terms were already described in the main paper). We would prefer to keep this Appendix as short as possible, as the rest of the technical details on how the method closes the equation (entirely derived from the references already quoted in the paper) is going to be repeated once more in a forthcoming paper, in preparation and more dedicated to the solver itself. 


R: Line 318: The mass ratio depends on what and how it affects the final results? Can you add a comment on this?  
A: While this is a parameter we cannot obviously vary in this cosmological simulation, we can use the results in the literature to guess the dependence on the mass ratio. For example, based on Cassano \& Brunetti 2005 (MNRAS), we can see that a 1:5 merger ratio is expected to inject about half of the total turbulent energy (normalised for the thermal gas energy) of a 1:2 merger ratio.  Based on this, it is likely that more rare 1:2 major mergers can produce even more efficient and longer-lasting re-acceleration of electrons and diffuse radio emission. However, this is the result of a semi-analytical treatment of the injection of turbulence in merger based on ram-pressure stripping, which neglects the associated dissipation of energy via shocks, and their related additional injection of particles via DSA. So only with  full simulations and a larger sample of simulated clusters it will be possible to assess in detail how the mass ratio of mergers result into different levels of particle-acceleration, in the scenario explored in this paper and in the so far little explored environment of MegaRH. We added a comment on this important issue in the revised  paper (Sec.4). 

R: 11-12 GYears, significant turbulence – efficient acceleration? However, from the plots, it seems that this is not supported. 
A: We added a more extended comment about this at the end of the Subsection. 


R: Line 369: Can the authors also provide the total energy number to clarify what fraction goes to the turbulent kinetic energy?  
A: Fixed, the numbers are reported at the end of the paragraph.

R: Line 385: What is the number of the significant fraction?  
A: Fixed. 

R: Line 517: Typo with an extra ) 
A: Fixed. 

R:  Line 597: Define R_{200}​ 
A: Fixed with footnote 1 as before. 

R:  Line 615: What is the value of the Mach number? 
A:  The turbulent Mach number is in the 0.2-0.3 range; we add a comment with more detailed measurements of this in the revised Sec.3.4

R:  Line 661: Define σ_ν​. 
A:  Fixed.

R:  Line 700: Do the authors consider the SSA, and what exactly is the inclination of the spectra? Can this be related to Fig. 8 and the differences between lower and higher frequencies? 
A: At the density of the intracluster medium and at the frequencies of interest here,  the spectrum is  dominated by orders of magnitude by the synchrotron flux and SSA is irrelevant at these frequencies, i.e. the radio photons emitted by synchrotron travel through an optically thin medium, hence this effect is entirely neglected. In the context of ICM studies, this circumstance is generally known, and we thought it was not necessary to add this detail to our presentation. 

R:  Figures:
>General Comment: In the figures sub-labels should be added for and easy reference (e.g., 1a, 1b, 2a, 2b, etc.). Then the authors can use them in the text as well to help the reader. Avoid the same type of line, e.g., Fig. 1, Fig. 5, Fig. 9.
A: Fixed. 

R:  Figure 2: Are these the same snapshots as in Fig. 1? It might be better to have the values in Gyr. Are the differences between CT and CST based on fluctuations? Does the shock-acceleration part impact the resolution? In general, DSA and turbulence do not have different results. In specific snapshots, e.g., z=0.27, the DSA is one order of magnitude more efficient.
A: Yes, we have now redone the caption of all plots to show the consistency of all used epochs. 



R: >Figure 3: Are e_{cr}/e_k​ normalized to an initial value for each quantity? The fourth plot does not have values on the x-axis. 
A: No, the number of tracers is not normalised but it represents the exact number of Lagrangian particles present in the region between 450 and 900 kpc. The number of tracers slightly increases after 2 Gyr,  within this radial selection, as result of the merger ejecting gas from the very centre.


R: Figure 5: In the third row, in the third figure, a tiny peak appears later. It may be better to delete it. 
A: Actually, this is just a local peak of the radio spectral index, which gets just at the level of -2.25 at about r=1300kpc at that epoch. 

R: Figure 6: Is the linear fit the best? It seems to be a broken power law. Which color is which one? The labels confuse the reader (not the Classical and MegaRH region)—the same for Fig. 7. 
A: The fit procedure, which basically wants to mimic the observational procedure, so far used on a handful of objects, is described in Section 3.3, which we have now further expanded to make it more readable. The procedure uses and exponential fit which takes into account for the central decrease of brightness due to the radial averaging of the SB. This is the best profile to describe the shape of the observed classical radio halos.


R:  Figure 9: Why don't the authors use the same timesteps as in the other plots/maps? Is it related to the merger between ~8 and ~9 Gyr? We expect to have a difference between 8.49 and 8.85 Gyr.
A: We chose to inject our spectra before or after major events such as the formation of the cluster (which is at about 8.6 Gyr) or the major merger (at about 12 Gyr). This helped us understand the evolution of the spectra with stochastic re-acceleration due to turbulence. Electrons indeed lose the "memory" of their initial energy, as evidenced by the distributions matching after a short time.
We commented on this in the caption of Fig.9, and in the related discussion. 

 


=================

Before resubmitting your manuscript, please take the time to verify the following common language and formatting issues.

1) Please note the spelling convention (US or UK) of your paper and run a spell check specific to your preference (see the A&A language guide for authors, Sect. 2.1, for common spelling and punctuation differences between these two conventions).
2) Check that abbreviations and acronyms are introduced correctly (see Sect. 5.2.4).
3) Check your reference format (see Sect. 3.6.2).

